General dynamic recovery for compensating CSP

Compensation is a technique to roll-back a system to a consistent state in case of failure. Recovery mechanisms for compensating calculi specify the order of execution of compensation sequences. Dynamic recovery means that the order of execution is determined at runtime. In this paper, we define an extension of Compensating CSP, called DEcCSP, with general dynamic recovery. We provide a formal, operational semantics for the calculus, and illustrate its expressive power with a case study. In contrast with previous versions of Compensating CSP, DEcCSP provides mechanisms to replace or discard compensations at runtime. Additionally, we bring back to DEcCSP standard CSP operators that are not available in other compensating CSP calculi, and introduce channel communication.

==> eptcsdata.tex <==
\providecommand{\firstpage}{3}
\providecommand{\publicationstatus}{B. L\"owe, G. Winskel (Eds.):\\
Developments in Computational Models 2012 (DCM 2012)\\
EPTCS 143, 2014, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.143.1}{10.4204/EPTCS.143.1}}

